Exploring the Phase Diagram of the quantum one-dimensional ANNNI model

This work presents a circuit-level integration of Quantum Machine Learning and Tensor Networks in the context of the one-dimensional Axial Next-Nearest-Neighbor Ising model with a transverse field. The study concretely connects these two paradigms: ground states of the model are obtained via the density matrix renormalization group as Matrix Product States and converted into quantum circuits, which are then used as input to a hybrid quantum-classical classifier and a Quantum Autoencoder by prepending the state-preparation circuit to the trainable ansatz. This construction directly addresses a key bottleneck of purely quantum workflows, namely the need for expensive, gradient-based optimization on hardware for every input state, by delegating state preparation to classical Tensor Network methods, which are scalable by construction. The result is a scalable and hardware-compatible pipeline for the task of studying spin systems.

==> tikz/circuits/brick4d2.tex <==
\definecolor{b4d2inputcolor}{HTML}{0096FF}
\begin{quantikz}[row sep={0.6cm,between origins}, column sep={.9cm,between origins}, background color=b4d2inputcolor!20]
	\lstick{$|0\rangle$} & \gate[2]{U^1_1} &                 &                 & [.2cm] \gate[2]{U^2_1} &                 &                 & \ldots \\
	\lstick{$|0\rangle$} &                 & \gate[2]{U^1_2} &                 &                        & \gate[2]{U^2_2} &                 & \ldots \\
	\lstick{$|0\rangle$} &                 &                 & \gate[2]{U^1_3} &                        &                 & \gate[2]{U^2_3} & \ldots \\
	\lstick{$|0\rangle$} &                 &                 &                 &                        &                 &                 & \ldots
\end{quantikz}

==> tikz/schema/anomaly4.tex <==
\def\autoencodersmallgroup{
	\gategroup[4,steps=11,style={dashed,rounded
				corners,fill=yellow!20, inner
				xsep=2pt},background,label style={label
				position=below,anchor=north,yshift=-0.2cm}]{}
}
\def\autoencodersmallgate{
	\gate[1][.6cm][.6cm]{}
}

\def\brickfoursmallgate{\gate[2][\brickfoursmallgatewidth]{}}
\begin{quantikz}[row sep={0.6cm,between origins}, column sep={.5cm,between origins}]
	 & \autoencodersmallgate\autoencodersmallgroup & [.1cm] \qw & \ctrl{1}  & [.1cm] \autoencodersmallgate & [.1cm] \qw & \qw       & \ctrl{2}  & [.1cm] \autoencodersmallgate & \qw & [-.5cm] \qw                                 & \\
	 & \autoencodersmallgate                       & \ctrl{1}   & \targ{-1} & \autoencodersmallgate        & \ctrl{1}   & \targ{2}  & \qw       & \autoencodersmallgate        & \qw & \rstick{\rule{.7cm}{0pt}$\langle Z\rangle$} & \\
	 & \autoencodersmallgate                       & \control{} & \targ{1}  & \autoencodersmallgate        & \control{} & \qw       & \targ{-2} & \autoencodersmallgate        & \qw & \rstick{\rule{.7cm}{0pt}$\langle Z\rangle$} & \\
	 & \autoencodersmallgate                       & \qw        & \ctrl{-1} & \autoencodersmallgate        & \qw        & \ctrl{-2} & \qw       & \autoencodersmallgate        & \qw & \qw                                         &
\end{quantikz}

==> tikz/schema/boxes/an.tex <==
\begin{tikzpicture}
	\pgfdeclarelayer{background}
	\pgfsetlayers{background,main}

	\node[draw, minimum width=4.5cm, minimum height=3cm] (boxx) {};
	\useasboundingbox (boxx.north west) rectangle (boxx.south east);

	\begin{pgfonlayer}{background}
		\fill[qtigreen!20]
		(boxx.north west)
		rectangle
		([yshift=-.5cm]boxx.north east);
	\end{pgfonlayer}

	\node[anchor=north, font=\bfseries] at (boxx.north) {Quantum Autoencoder};

	\node (mps) at ([yshift=-.2cm]boxx.center) {
		\scalebox{.6}{\input{tikz/schema/anomaly4.tex}}
	};

\end{tikzpicture}

==> tikz/schema/boxes/brick.tex <==
\begin{tikzpicture}
	\pgfdeclarelayer{background}
	\pgfsetlayers{background,main}

	% Main box
	\node[draw, minimum width=3.75cm, minimum height=2.5cm] (boxx) {};

	% Background layer
	\begin{pgfonlayer}{background}
		\fill[qtiteal!20]
		(boxx.north west)
		rectangle
		([yshift=-.5cm]boxx.north east);
	\end{pgfonlayer}

	% Title
	\node[anchor=north, font=\bfseries] at (boxx.north) {Brick Ansatz};

	% Brick graphic
	\node (mps) at ([yshift=-.2cm]boxx.center) {
		\input{tikz/schema/brick4.tex}
	};

\end{tikzpicture}

==> tikz/schema/boxes/dmrg.tex <==
\begin{tikzpicture}
	\pgfdeclarelayer{background}
	\pgfsetlayers{background,main}

	% Main box
	\node[draw, minimum width=3.5cm, minimum height=2.5cm] (dmrg) {};

	% Background layer
	\begin{pgfonlayer}{background}
		\fill[qtiblue!20]
		(dmrg.north west)
		rectangle
		([yshift=-.5cm]dmrg.north east);
	\end{pgfonlayer}

	% Title
	\node[anchor=north, font=\bfseries] at (dmrg.north)
	{DMRG Algorithm};

	% MPS graphic
	\node[anchor=west] (mpslabel) at ([yshift=.5cm]dmrg.west)
	{Ground state:};
	\node (mps) at ([yshift=-.2cm]dmrg.center)
	{\rotatebox{-90}{\input{tikz/schema/mps4.tex}}};

	% Label
	\node[below] at (mps.south) {Matrix Product State};

\end{tikzpicture}

==> tikz/schema/boxes/hc.tex <==
\begin{tikzpicture}
	\pgfdeclarelayer{background}
	\pgfsetlayers{background,main}

	\node[draw, minimum width=4.5cm, minimum height=3cm] (boxx) {};
	\useasboundingbox (boxx.north west) rectangle (boxx.south east);

	\begin{pgfonlayer}{background}
		\fill[qtigreen!20]
		(boxx.north west)
		rectangle
		([yshift=-.5cm]boxx.north east);
	\end{pgfonlayer}

	\node[anchor=north, font=\bfseries] at (boxx.north) {Hybrid Classifier};

	\node (mps) at ([xshift=-.2cm, yshift=-.3cm]boxx.center) {
		\scalebox{.6}{\input{tikz/schema/hc4.tex}}
	};

\end{tikzpicture}


==> tikz/schema/brick4.tex <==
\definecolor{brick4color}{HTML}{0096FF}
\def\brickfoursmallgatewidth{0.4cm}
\def\brickfoursmallgate{%
	\gate[2, style={fill=brick4color!20}]{}%
}

\begin{quantikz}[row sep={0.45cm,between origins}, column sep={.45cm,between origins}]
	\lstick{$|0\rangle$} & \brickfoursmallgate & \qw                 & \qw                 & [-.25cm] \brickfoursmallgate & \qw                 & \qw                 & [-.25cm] \ldots \\
	\lstick{$|0\rangle$} & \qw                 & \brickfoursmallgate & \qw                 & \qw                          & \brickfoursmallgate & \qw                 & \ldots          \\
	\lstick{$|0\rangle$} & \qw                 & \qw                 & \brickfoursmallgate & \qw                          & \qw                 & \brickfoursmallgate & \ldots          \\
	\lstick{$|0\rangle$} & \qw                 & \qw                 & \qw                 & \qw                          & \qw                 & \qw                 & \ldots
\end{quantikz}

==> tikz/schema/hc4.tex <==
\def\hcboxheight{3.1cm}
\def\hcsmallgroup{
	\gategroup[4,steps=9,style={dashed,rounded
				corners,fill=red!20, inner
				xsep=2pt,minimum height=\hcboxheight},background,label style={label
				position=below,anchor=north,yshift=-0.2cm}]{}
}
\def\hcsmallgate{
	\gate[1][.6cm][.6cm]{}
}

\begin{tikzpicture}
	\pgfdeclarelayer{background}
	\pgfsetlayers{background,main}
	\node (circuit) {%
		\begin{quantikz}[row sep={0.6cm,between origins}, column sep={.5cm,between origins}]
			 & \hcsmallgate\hcsmallgroup & \ctrl{1}   & \hcsmallgate & \qw        & \hcsmallgate & \ctrl{1}   & \hcsmallgate & \qw        & [-.25cm] \qw \\
			 & \hcsmallgate              & \control{} & \hcsmallgate & \ctrl{1}   & \hcsmallgate & \control{} & \hcsmallgate & \ctrl{1}   & \qw          \\
			 & \hcsmallgate              & \ctrl{1}   & \hcsmallgate & \control{} & \hcsmallgate & \ctrl{1}   & \hcsmallgate & \control{} & \qw          \\
			 & \hcsmallgate              & \control{} & \hcsmallgate & \qw        & \hcsmallgate & \control{} & \hcsmallgate & \qw        & \qw
		\end{quantikz}
	};
	\begin{scope}[shift={($(circuit.east)+(.25cm,.12cm)$)}]
		\foreach \i/\y in {1/0.9,2/0.3,3/-0.3,4/-0.9}
		\node[circle, draw, fill=white, minimum size=7pt, inner sep=0pt] (in\i) at (0,\y) {};
		\foreach \i/\y in {1/0.8,2/0.4,3/0,4/-0.4,5/-0.8}
		\node[circle, draw, fill=white, minimum size=7pt, inner sep=0pt] (hid\i) at (0.7,\y) {};
		\foreach \i/\y in {1/0.4,2/0,3/-0.4}
		\node[circle, draw, fill=white, minimum size=7pt, inner sep=0pt] (out\i) at (1.4,\y) {};

		\foreach \i in {1,...,4}
		\foreach \j in {1,...,5}
		\draw[gray, thin] (in\i) -- (hid\j);
		\foreach \j in {1,...,5}
		\foreach \k in {1,...,3}
		\draw[gray, thin] (hid\j) -- (out\k);

		\begin{pgfonlayer}{background}
			\node[draw, dashed, rounded corners, thick, fill=green!20, fit=(in1)(in4)(hid1)(hid5)(out1)(out3), inner sep=7pt, minimum height=\hcboxheight] (nnbox) {};
		\end{pgfonlayer}
	\end{scope}
\end{tikzpicture}

==> tikz/schema/mps4.tex <==
\definecolor{mps4color}{HTML}{0096FF}
\newcommand{\mpsspin}{
	\begin{tikzpicture}
		% filled circle with thick black outline (center fixed at origin)
		\node[draw=black, thick, circle, minimum size=.3cm, inner sep=0pt, fill=mps4color!20 ] (c) at (0,0) {};

	\end{tikzpicture}
}
\begin{tikzpicture}
	\def\spindist{.6cm}
	\def\spinout{.4cm}
	% Declare layers
	\pgfdeclarelayer{background}
	\pgfsetlayers{background,main}

	% Spins
	\node (spin1) at (0, 0) {\mpsspin};
	\node (spin2) at ([yshift=-\spindist]spin1) {\mpsspin};
	\node (spin3) at ([yshift=-\spindist]spin2) {\mpsspin};
	\node (spin4) at ([yshift=-\spindist]spin3) {\mpsspin};

	% Line in the background layer
	\begin{pgfonlayer}{background}
		% connection between spins
		\draw[thick] (spin1.center) -- (spin4.center);

		% spin to out
		\draw[thick] (spin1.center) -- ([xshift=\spinout]spin1.center);
		\draw[thick] (spin2.center) -- ([xshift=\spinout]spin2.center);
		\draw[thick] (spin3.center) -- ([xshift=\spinout]spin3.center);
		\draw[thick] (spin4.center) -- ([xshift=\spinout]spin4.center);
	\end{pgfonlayer}
\end{tikzpicture}
